On the Sublinear Regret of GP-UCB

In the kernelized bandit problem, a learner aims to sequentially compute the optimum of a function lying in a reproducing kernel Hilbert space given only noisy evaluations at sequentially chosen points. In particular, the learner aims to minimize regret, which is a measure of the suboptimality of the choices made. Arguably the most popular algorithm is the Gaussian Process Upper Confidence Bound (GP-UCB) algorithm, which involves acting based on a simple linear estimator of the unknown function. Despite its popularity, existing analyses of GP-UCB give a suboptimal regret rate, which fails to be sublinear for many commonly used kernels such as the Mat\'ern kernel. This has led to a longstanding open question: are existing regret analyses for GP-UCB tight, or can bounds be improved by using more sophisticated analytical techniques? In this work, we resolve this open question and show that GP-UCB enjoys nearly optimal regret. In particular, our results yield sublinear regret rates for the Mat\'ern kernel, improving over the state-of-the-art analyses and partially resolving a COLT open problem posed by Vakili et al. Our improvements rely on a key technical contribution -- regularizing kernel ridge estimators in proportion to the smoothness of the underlying kernel $k$. Applying this key idea together with a largely overlooked concentration result in separable Hilbert spaces (for which we provide an independent, simplified derivation), we are able to provide a tighter analysis of the GP-UCB algorithm.

==> old_tex/Determinant_Rate.tex <==
\section{Improved Regret via Method of Mixtures}

In this section, we present an improved regret analysis for the Gaussian Process UCB algorithm, as outlined in Algorithm~\ref{alg:UCB} above. Our key insights in our analysis are as follows. First, we observe that, by making a careful truncation argument, one can reduce self-normalized in an RKHS to self-normalized concentration in finite-dimensional Euclidean space. In particular, we provide a time-uniform, self-normalized concentration bound that improves on that of \citet{chowdhury2017kernelized} in terms of both generality and tightness. Our second contribution is recognizing the importance of regularization in the GP-UCB algorithm. Existing analyses essentially assume the regularization parameter $\rho$ to be constant. We show that significant improvements to regret can be obtained when $\rho$ is chosen to reflect (a) the time horizon $T$, (b) the dimensionality $d$, and (c) the overall smoothness of the functions produced by the kernel $k$.

With these insights, we are able to make the following improvement to the GP-UCB algorithm. 

\begin{theorem}
\label{thm:det_ucb}
Let $T > 0$ be a fixed time horizon, and let $\rho_T > 1$ be an arbitrary regularization parameter. Suppose we run GP-UCB (Algorithm~\ref{alg:UCB}) with inputs $\rho_T, T,$ and confidence bounds $(U_t)_{t \geq 0}$ given by
$$
U_t := \sqrt{2\log\left(\frac{\sqrt{\det(\rho^{-1}_TV_t)}}{\delta}\right)} + \rho_T^{1/2}D.
$$

Then, GP-UCB attains regret
\begin{align*}
R_T &\leq 2\left(\sqrt{2(\gamma_T(\rho_T) + \log(1/\delta))} + \rho^{1/2}D\right)\sqrt{2T\gamma_T(\rho_T)} \\
&= O\left(\gamma_T(\rho_T)\sqrt{T} + \sqrt{\rho_T\gamma_T(\rho_T)T}\right),
\end{align*}
where in the big-Oh notation above we treat $\delta$ and $D$ as being held constant. 

In particular, if the underlying kernel $k$ experiences $(C, \beta)$-polynomial eigendecay for some $C > 0$ and $\beta > 1$, we have the regret bound
$$
R_T = \widetilde{O}\left(T^{\frac{1}{1 + \beta} + \frac{1}{2}}\right) = \widetilde{O}\left(T^{\frac{3 + \beta}{2 + 2\beta}}\right),
$$
which is always sub-linear in $T$.


\end{theorem}

In the case of the Mat\'ern family of kernels, we have the following.

\begin{corollary}
Assume the same setup as Theorem~\ref{thm:det_ucb} above. Further, suppose the underlying kernel function $k$ is taken to be the $(\nu, \sigma)$-Mat\'ern kernel for some bandwidth $\sigma$ and some smoothness parameter $\nu > \frac{1}{2}$. Then GP-UCB attains 
$$
R_T = \widetilde{O}\left(T^{\frac{\nu + 2d}{2\nu + 2d}}\right)
$$
with high-probability.
\end{corollary}
Note that the above regret rate is sublinear for all $\nu > \frac{1}{2}$, which was not the case for the existing regret analysis done by \citet{chowdhury2017kernelized}, in which the regret guarantee of GP-UCB failed to even be sublinear. Further, observe that the regret rate provided by the above corollary is not far off from the optimal rate of $R_T$, which is $ \widetilde{O}\left(T^{\frac{\nu + d}{2\nu + d}}\right)$, showing that GP-UCB is nearly optimal.

To show the above result, we begin by proving the following self-normalized martingale concentration result for RKHS's. The following result can be viewed as a direct analogue of the method of {\color{red}incomplete sentence}


\begin{theorem}
    Suppose $(S_t)_{t \geq 0}$ is a non-negative martingale in a reproducing kernel Hilbert space $(H, (\cdot, \cdot)_H)$ with respect to some filtration $(\calF_t)_{t \geq 0}$. Further, suppose $(V_t)_{t \geq 0}$ is an $(\calF_t)_{t \geq 0}$-adapted process of positive-definite, finite rank linear operators $V_t : H \rightarrow H$ such that, for any $\lambda \in H$, the process
    $$
    \exp\left\{(\lambda, S_t)_H - \frac{1}{2}\lambda^T V_t \lambda \right\} 
    $$
    is a non-negative supermartingale with respect to $(\calF_t)_{t \geq 0}$, where $\lambda^T V_t \lambda := (V_t \nu, \nu)_H = (\nu, V_t \nu)_H$. Then, for any $\rho > 0$, we have, with probability at least $1 - \delta$, simultaneously for all $t \geq 0$
    $$
    \|V_t^{-1/2}S_t\|_H \leq \sigma\sqrt{2\log\sqrt{\det(\id_H + \rho^{-1}V_t)} + \log\left(\frac{1}{\delta}\right)}.
    $$
\end{theorem}

\begin{proof}

    Define the $(\calF_t)_{t \geq 0}$-adapted process $(X_t)_{t \geq 0}$ to be 
    $$
    X_t := \frac{1}{\sqrt{\det(\id_H + \rho^{-1}V_t)}}\exp\left\{\frac{1}{2}\left\|V_t^{-1/2}S_t\right\|^2\right\}
    $$
    with $X_0 := 1$. It suffices to show that $(X_t)_{t \geq 0}$ is a non-negative supermartingale with respect to $(\calF_t)_{t \geq 0}$, as Ville's inequality will yield that, for any $\delta \in (0, 1)$, simultaneously for all $t \geq 0$,
    $$
    \frac{1}{\sqrt{\det(\id_H + \rho^{-1}V_t)}}\exp\left\{\frac{1}{2}\left\|V_t^{-1/2}S_t\right\|^2\right\} \leq \frac{1}{\delta},
    $$
    i.e. after rearranging
    $$
    \left\|V_t^{-1/2}S_t\right\|_H \leq \sqrt{2\log\left(\frac{\sqrt{\det(\id_H + \rho^{-1}V_t)}}{\delta}\right)}.
    $$
    
    We argue that this process $(X_t)_{t \geq 0}$ is  a non-negative supermartingale in the following way. First, we truncate $(S_t)_{t \geq 1}$ into a finite-dimensional process by projecting onto a finite number of basis functions for the RKHS $H$. Then, we leverage an isometry between this finite-dimensional subspace and Euclidean space to apply the method of mixtures to obtain a non-negative supermartingale. Lastly, we make a limiting argument to show that the non-negative supermartingale approaches $(X_t)_{t \geq 0}$.

    For $n \geq 1$, define the functions $\varphi_n := \sqrt{\mu_n}\phi_n$. Observe that the system $(\varphi_n)_{n \geq 1}$ forms an orthonormal basis for $H$ under inner product $(\cdot, \cdot)_H$. Further, we can represent $H$ with respect to these basis functions as
    $$
    H = \left\{f = \sum_{n = 1}^\infty \beta_n \varphi_n : \sum_{n = 1}^\infty \beta_n^2 < \infty\right\}.
    $$
    In particular, this representation yields a natural isometric isomorphism between the spaces $H$ and $\ell^2(\N)$ given by
    $$
    f = \sum_{n = 1}^\infty\beta_n \varphi_n \mapsto (\beta_n)_{n \geq 1}.
    $$

    Let us refer to the above isometric isomorphism as $T$. Letting $H_n := \mathrm{span}(\varphi_1, \dots, \varphi_n)$, we can define the projection operator $\pi : H \rightarrow H_n$ as
    $$
    \pi_n f := \sum_{k = 1}^n (f, \varphi_k) \varphi_k.
    $$
    Observe that, for any $n$, any operator $A : H \rightarrow \ell^2(\N)$ restricts naturally to an operator $A|_n : H_n \rightarrow \R^n$. In particular, $T$ restricts to a natural isometric isomorphism $T_n : H_n \rightarrow \R^n$ given by $T_n f := (\beta_1, \dots, \beta_n)$, where we assume $f = \sum_{m =1}^n \beta_m \varphi_m$.

    By the assumption of the theorem, we know that for any $\lambda \in H_n$, the process
    $$
    \exp\left\{(\lambda, S_t)_H - \frac{1}{2}\lambda^T V_t \lambda\right\} = \exp\left\{(\lambda, S_t)_H - \frac{1}{2}(\lambda, V_t\lambda)_H\right\}
    $$
    is a non-negative supermartingale with respect to $(\calF_t)_{t \geq 0}$. In particular, for any probability measure $\mu$ on $\R^n$, it follows from Fubini's theorem that the ``mixture'' process $(X_t^{(n)})_{t \geq 0}$ given by
    $$
    X_t^{(n)} := \int_{H_n}\exp\left\{(\lambda, S_t)_H - \frac{1}{2}\lambda^TV_t\lambda\right\}\mu(d\lambda)
    $$
    is also a non-negative supermartingale with respect to $(\calF_t)_{t \geq 0}$. Now, let $\mu$ be the law of the random function $\Lambda := \sum_{m = 1}^n \xi_n \varphi_n$, where $\xi_1, \dots, \xi_n$ are i.i.d. $\calN(0, \rho)$ random variables. Further, let $f_\rho$ denote the density of a $\calN(0, \rho I_n)$ random variable. We have that
    \begin{align*}
    X_t^{(n)} &= \int_{H_n}\exp\left\{(\lambda, S_t)_H - \frac{1}{2}(\lambda, V_t\lambda)_H\right\}\mu(d\lambda) \\
    &= \int_{H_n}\exp\left\{(\lambda, \pi_nS_t)_H - \frac{1}{2}(\lambda, \pi_nV_t\lambda)_H\right\}\mu(d\lambda)\\
    &= \int_{H_n} \exp\left\{\langle T_n\lambda, T_n \pi_nS_t\rangle - \frac{1}{2}\langle T_n\lambda, T_n\pi_nV_t\lambda\rangle \right\}\mu(d\lambda) \\
    &= \int_{\R^n}\exp\left\{\langle\widehat{\lambda}, T_n\pi_nS_t\rangle - \frac{1}{2}\langle \widehat{\lambda}, T_n\pi_nV_t\pi_nT_n^{-1}\widehat{\lambda}\rangle \right\}f_\rho(\widehat{\lambda})d\widehat{\lambda} \\
    &= \int_{\R^n}\exp\left\{\widehat{\lambda}^T(T_n\pi_nS_t) - \frac{1}{2}\widehat{\lambda}^T\left(T_nV_t^{(n)}T_n^{-1}\right)\widehat{\lambda}\right\}f_\rho(\widehat{\lambda})d\widehat{\lambda} \\
    &= \int_{\R^n}\exp\left\{\widehat{\lambda}^T\calS_t^{(n)} - \frac{1}{2}\widehat{\lambda}^T\calV_t^{(n)}\widehat{\lambda}\right\}f_\rho(\widehat{\lambda})d\widehat{\lambda} \\
    &= \left(\det(I_n + \rho^{-1}\calV_t^{(n)}) + \rho I_n\right)^{-1/2}\exp\left\{\frac{1}{2}\left\|\left(\calV_t^{(n)}\right)^{-1/2}\calS_t^{(n)}\right\|^2\right\}\\
    &=\left(\det(\id_H + \rho^{-1}\pi_nV_t\pi_n)\right)^{-1/2}\exp\left\{\frac{1}{2}\left\|\left(T_n\pi_n(V_t + \rho\id_H)\pi_nT_n^{-1}\right)^{-1/2}T_n\pi_nS_t\right\|^2\right\} \\
    &= \left(\det(\id_H + \rho^{-1}\pi_nV_t\pi_n)\right)^{-1/2}\exp\left\{\frac{1}{2}\left\|T_n\pi_n(V_t + \rho\id_H)^{-1/2}\pi_nS_t\right\|^2\right\} \\
    &=\left(\det(\id_H + \rho^{-1}\pi_nV_t\pi_n)\right)^{-1/2}\exp\left\{\frac{1}{2}\left\|\pi_n (V_t + \rho\id_H)^{-1/2} \pi_nS_t\right\|_H^2\right\}.
    \end{align*}

    We now argue $X_t^{(n)} \rightarrow X_t$ as $n \rightarrow \infty$ almost surely. First, it is clear that, for any $f \in H$, we have $\pi_n f \rightarrow f$ in $H$ as $n \rightarrow \infty$, i.e. $\|f - \pi_n f\|_H \rightarrow 0$ as $n \rightarrow \infty$. Next, since $V_t$ is assumed to be of finite rank, it further follows that $\|(V_t + \rho\id_H)^{-1/2}(\pi_n - \id_H)\|_{op} \rightarrow 0$ and $\|V_t(\pi_n - \id_H)\|_{op} \rightarrow 0$ as $n \rightarrow \infty$, where $\|\cdot\|_{op}$ denotes the operator norm on $H$ with respect to $\|\cdot\|_H$, i.e. if $A : H \rightarrow H$ is an operator, then $\|A\|_{op} := \sup_{\|f\|_H = 1}\|Af\|_H$. 

    From these observations, it follows that $\|\pi_n V_t \pi_n - V_t\|_{op} \rightarrow 0$ as $n \rightarrow \infty$. Since $\det(\id_H + A)$ is continuous under Trace-norm $\|A\|_1 := Tr(\|A\|)$, and since 
    $$
    \|\pi_nV_t\pi_n - V_t\|_1 \leq 2t \|\pi_nV_t\pi_n - V_t\|_{op} \rightarrow 0 \quad \text{as } n \rightarrow \infty,
    $$
    we have 
    $$
    \left(\det(\id_H + \rho^{-1}\pi_nV_t\pi_n)\right)^{-1/2} \xrightarrow[n \rightarrow \infty]{} \left(\det(\id_H + \rho^{-1}V_t)\right)^{-1/2}.
    $$
    Likewise, we have by a similar argument that
    $$
    \left\|\pi_n(V_t + \rho \id_H)^{-1/2}\pi_nS_t\right\|_H \rightarrow  \left\|(V_t + \rho\id_H)^{-1/2}S_t\right\|_H \quad \text{as } n \rightarrow \infty.
    $$
    Thus, we have the desired almost sure convergence that $X_t^{(n)} \rightarrow X_t$ as $n \rightarrow \infty$. Now, using this convergence, we can show $(X_t)_{t \geq 0}$ is a non-negative supermartingale with respect to $(\calF_t)_{t \geq 0}$. In particular, by Fatou's lemma, we have
    \begin{align*}
    \E(X_t \mid \calF_{t - 1}) &= \E(\liminf_{n \rightarrow \infty}X_t^{(n)} \mid \calF_{t - 1})\\
    &\leq \liminf_{n \rightarrow \infty}\E(X_t^{(n)} \mid \calF_{t - 1}) \\
    &\leq \liminf_{n \rightarrow \infty}X_{t - 1}^{(n)} \\
    &= X_{t  -1}.
    \end{align*}
    Thus, we have proved the desired result and are done.

\end{proof}

With the above theorem, the proof of Theorem~\ref{thm:det_ucb} is straightforward. 

\begin{proof}
Observe that, using standard techniques, we can bound the instantaneous regret $r_t$ as
\begin{align*}
    r_t &:= f^\ast(x^\ast) - f^\ast(X_t) = \left(f^\ast, k(\cdot, x^\ast)\right)_H - \left(f^\ast, k(\cdot, X_t)\right)_H \\
    &\leq \left(\widetilde{f}_{t - 1}, k(\cdot, X_t)\right)_H - \left(f^\ast, k(\cdot, X_t)\right)_H \\
    &= \left(\widetilde{f}_{t - 1} - \widehat{f}_{t - 1}, k(\cdot, X_t)\right)_H + \left(\widehat{f}_{t - 1} - f^\ast, k(\cdot, X_t)\right)_H \\
    &\leq \left\|V_{t - 1}^{-1/2}k(\cdot, X_t)\right\|_H\left\|V_{t - 1}^{1/2}(\widetilde{f}_{t - 1} - \widehat{f}_{t - 1})\right\|_H + \left\|V_{t - 1}^{-1/2}k(\cdot, X_t)\right\|_H\left\|V_{t - 1}^{1/2}(\widehat{f}_{t - 1} - f^\ast)\right\|_H \\
    &\leq 2\left\|V_{t - 1}^{-1/2}k(\cdot, X_t)\right\|_H\left(\sqrt{2\log\left(\frac{\sqrt{\det(\rho^{-1}_T V_{t - 1})}}{\delta}\right)} + \rho^{1/2}_T\|f^\ast\|_{H}\right)\\
    &\leq 2\left\|V_{t - 1}^{-1/2}k(\cdot, X_t)\right\|_H\left(\sqrt{2(\gamma_{t - 1}(\rho_T) + \log(1/\delta))} + \rho^{1/2}_T\|f^\ast\|_H\right) \\
    &\leq 2\left\|V_{t - 1}^{-1/2}k(\cdot, X_t)\right\|_H\left(\sqrt{2(\gamma_T(\rho_T) + \log(1/\delta))} + \rho^{1/2}_T\|f^\ast\|_H\right).
\end{align*}

Consequently, applying Cauchy-Schwarz to regret yields
\begin{align*}
R_T &= \sum_{t = 1}^T r_t\\
&\leq 2\left(\sqrt{2(\gamma_T(\rho_T) + \log(1/\delta))} + \rho^{1/2}\|f^\ast\|_H\right)\sum_{t = 1}^T\left\|V_{t - 1}^{-1/2}k(\cdot, X_t)\right\|_H \\
&\leq 2\left(\sqrt{2(\gamma_T(\rho_T) + \log(1/\delta))} + \rho^{1/2}\|f^\ast\|_H\right)\sqrt{T\sum_{t = 1}^T \left\|V_{t - 1}^{-1/2}k(\cdot, X_t)\right\|_H^2} \\
&\leq 2\left(\sqrt{2(\gamma_T(\rho_T) + \log(1/\delta))} + \rho^{1/2}\|f^\ast\|_H\right)\sqrt{2T\log\det(\rho^{-1}_TV_T)} \\
&\leq 2\left(\sqrt{2(\gamma_T(\rho_T) + \log(1/\delta))} + \rho^{1/2}D\right)\sqrt{2T\gamma_T(\rho_T)} \\
&= O\left(\gamma_T(\rho_T)\sqrt{T} + \sqrt{\rho\gamma_T(\rho_T)T}\right).
\end{align*}

Now, assume that the the kernel $k$ experiences $(C, \beta)$-polynomial eigendecay, i.e. the sequence of eigenvalues $(\mu_n)_{n \geq 1}$ associated with the Hilbert-Schmidt operator $T_k$ satisfy $\mu_n \leq Cn^{-\beta}$ for all $n \geq 1$. Further, assume that the kernel $k$ satisfies the assumptions of Lemma~\ref{lem:info_gain_bound}. Then, there exists some constant $C'$ dependent only on $C, K, \psi,$ and $\beta$ such that
$$
\gamma_T(\rho_T) \leq \left(C'\left(\frac{T}{\rho_T}\right)^{1/\beta}\log^{-1/\beta}\left(1 + \frac{KT}{\rho_T}\right) + 1\right)\log\left(1 + \frac{KT}{\rho_T}\right).
$$
We now select $\rho_T$ to satisfy $\rho_T = \left(\frac{T}{\rho_T}\right)^{1/\beta}$, which can be checked to be true when $\rho_T = T^{\frac{1}{1 + \beta}}$. In this case, we have.
$$
\gamma_T(\rho_T) \leq \left(C'T^{\frac{1}{1 + \beta}}\log^{-1/\beta}(1 + KT^{\beta/(1 + \beta)}) + 1\right)\log(1 + KT^{\beta/(1 + \beta)})
$$
A similar calculation yields
$$
\sqrt{\rho_T\gamma_T(\rho_T)} \leq T^{\frac{1}{1 + \beta}}\sqrt{2C'\log^{-1/\beta}(1 + KT^{\beta/(1 + \beta)})\log(1 + KT^{\beta/(1 + \beta)})}.
$$
In particular, up to constant and polylogarithmic (in $T$) factors, we have equalized the terms $\gamma_T(\rho_T)$ and $\sqrt{\rho_T\gamma_T(\rho)}$, and have showed that
$$
\gamma_T(\rho_T) = \widetilde{O}\left(T^{\frac{1}{1 + \beta}}\right) \quad \text{and} \quad \sqrt{\rho_t\gamma_T(\rho_T)} = \widetilde{O}\left(T^{\frac{1}{1 + \beta}}\right).
$$
Thus, applying our previous regret analysis, we see that
$$
R_T \leq \widetilde{O}\left(T^{\frac{1}{1 + \beta} + \frac{1}{2}}\right),
$$
which, in particular, is sublinear for any $\beta > 1$.
\end{proof}


==> old_tex/background.tex <==
\section{Background on Reproducing Kernel Hilbert Space Theory}

In this section, we discuss the basics of reproducing kernel Hilbert space (or RKHS) theory. We start 

\subsection{Basics of RKHS's}

Let $\calX \subset \R^d$ be a bounded, compact set. We say a function $k : \calX \times \calX \rightarrow \R$ is \textbf{positive semi-definite} if, for any $n \in \N$ and $x_1, \dots, x_n$, the Gram matrix $\left(k(x_i, x_j)\right)_{i, j \in [n]}$ is positive semi-definite. Going forward, we call any such positive semi-definite function $k$ a \textbf{kernel function}.

Any kernel function $k$ can be associated with a unique \textbf{reproducing kernel Hilbert space} or \textbf{RKHS} $(H, (\cdot, \cdot)_H)$ satisfying $k(\cdot, x) \in H$ for each $x \in H$ and
$$
f(x) = (k(\cdot, x), f)_H \qquad \text{for all } f \in H.
$$
Explicitly, the space $H$ can be defined as the completion of the inner product space 
$$
H := \left\{ \sum_{n = 1}^N \alpha_n k(\cdot, x_n) : N \in \N, \alpha_1, \dots, \alpha_N \in \R, x_1, \dots, x_N \in \calX\right\} 
$$
under point-wise limits. We do not discuss this representation further as alternative representations will be more useful in the sequel. Going forward, we only concern ourselves with \textbf{translation-invariant kernels}, or kernels that can be written as $k(x, y) = k(\|x - y\|)$, where $\|\cdot\|$ denotes the standard Euclidean or $\ell_2$ norm on $\R^d$.

We discuss two families of translation-invariant kernel functions that are particularly useful in machine learning-related endeavors. First, there is the \textbf{squared-exponential} or \textbf{Gaussian kernel}, which for an arbitrary bandwidth parameter $\sigma > 0$ is given by
$$
k(x, y) = k(\|x - y\|) := \exp\left\{\frac{-\|x - y\|^2}{2\sigma^2}\right\}, \quad \text{for all } x, y \in \calX.
$$
Another useful family of translation-invariant kernels is the \textbf{Mat\'ern kernel} family. For a bandwidth parameter $\sigma > 0$ and a smoothness parameter $\nu > 0$, the corresponding Mat\'ern kernel is given by
$$
k(x, y) = k(\|x - y\|) := \frac{1}{\Gamma(\nu)2^{\nu - 1}}\left(\frac{\sqrt{2\nu}\|x - y\|}{\sigma}\right)^\nu B_\nu\left(\frac{\sqrt{2\nu}\|x - y\|}{\sigma}\right),\quad \text{for any } x, y \in \calX,
$$
where $\Gamma(z) := \int_0^\infty t^{z - 1}e^{-t}dt$ is the Gamma function, and $B_\nu(z)$ is the modified Bessel function of the second kind. The Mat\'ern family of kernels is often preferred over the squared exponential family in practical settings, as the smoothness parameter $\nu > 0$ gives increased expressivity. In particular, the squared exponential kernel can be recovered by sending $\nu \rightarrow \infty$.



\subsection{Representations of RKHS's}
In this section, we discuss an alternative, more informative representation of the RKHS $H$ in terms of the eigenfunctions and eigenvalues of the Hilbert-Schmidt operator associated with the underlying kernel $k$. 

Let $\mu$ be an arbitrary finite Borel measure on $\calX$ (where we view $\calX$ under the subspace topology and denote by $\calB(\calX)$ the corresponding Borel sets on $\calX$). We define the space of all square-integrable measurable functions $f : \calX \rightarrow \R$ on $(\calX, \calB(\calX), \mu)$ as
$$
L^2(\calX) = L^2(\calX, \calB(\calX), \mu) := \left\{ f : \calX \rightarrow \R \text{ measurable } : \int_\calX f(x)^2\mu(dx) < \infty\right\}.
$$
$L^2(\calX)$ can be made into a Hilbert space under the inner product $(\cdot, \cdot) : L^2(\calX) \times L^2(\calX) \rightarrow \R$ given by
$$
(f, g)_{L^2} := \int_\calX f(x)g(x)\mu(dx), \quad \text{for all } f, g \in L^2(\calX).
$$
If the kernel under consideration $k : \calX \times \calX \rightarrow \R$ is square-integrable in the sense that
$$
\int_\calX k(x, y)^2 \mu(dx) < \infty,
$$
one can define the corresponding \textbf{Hilbert-Schmidt operator} $T_k : L^2(\calX) \rightarrow L^2(\calX)$ by
$$
T_kf(x) := \int_\calX k(x, y) f(y)\mu(dx).
$$
Intuitively, $T_k$ can be viewed as smoothing out the function $f$ over the domain $\calX$ according the kernel $k$. The Hilbert-Schmidt operator $T_k$ plays an integral in RKHS theory through Mercer's theorem, which states the the RKHS $(H, (\cdot, \cdot)_H)$ associated with kernel $k$ can be defined explicitly in terms of the eigenfunctions and eigenvalues of $T_k$. We state this theorem below.

\begin{theorem}
\label{thm:mercer}
Suppose $\calX$ is compact and $k : \calX \times \calX \rightarrow \R$ is a continuous kernel function. Then, the eigenfunctions $(\phi_n)_{n \in \N}$ of $T_k$ form an orthonormal basis for $L^2(\calX)$ with corresponding non-negative eigenvalues $(\mu_n)_{n \in \N}$. Further, the RKHS $H$ is explicitly given by
$$
H = \left\{ f = \sum_{n \in \N}\beta_n \phi_n : \beta_n \in \R, \sum_{n \in \N}\frac{\beta_n^2}{\mu_n} < \infty\right\}.
$$
Further, the inner product $(\cdot, \cdot)_H : H \times H \rightarrow \R$ is given by
$$
(f, g)_H = \sum_{n \in \N}\mu_n^{-1}(f, \phi_n)_{L^2}(g, \phi_n)_{L^2}.
$$

\end{theorem}

For simplicity, we always assume the eigenfunctions $(\phi_n)_{n \in \N}$ associated with $T_k$ are indexed such that the corresponding sequence of eigenvalues $(\mu_n)_{n \in \N}$ is decreasing. Mercer's theorem is useful for our endeavors as it allows to view the RKHS $H$, a potentially complicated space of functions, as being isomorphic to an infinite-dimensional ellipsoid. More rigorously, let $\ell^2(\N)$ be the space of all square-convergent real-valued sequences, i.e.
$$
\ell^2(\N) := \left\{ \beta := (\beta_n)_{n \in \N} : \sum_{n \in \N}\beta_n^2 < \infty\right\}.
$$
$\ell^2(\N)$ itself is a Hilbert space under corresponding inner product $\langle \cdot, \cdot \rangle : \ell^2(\N) \times \ell^2(\N) \rightarrow \N$ given by $\langle \alpha, \beta \rangle := \sum_{n \in \N}\alpha_n\beta_n$. In other words, $\langle \cdot, \cdot \rangle$ is just the extension of standard Euclidean dot product to an infinite dimensional space. 

Of particular import to us is the infinite-dimensional subspace $\Epsilon \subset \ell^2(\N)$ given by
$$
\Epsilon := \left\{\beta \in \ell^2(\N) : \sum_{n \in \N} \frac{\beta_n^2}{\mu_n} < \infty\right\},
$$
where $(\mu_n)_{n \in \N}$ is the decreasing sequence of non-negative eigenvalues associated with some kernel $k$. $\Epsilon$ is itself a Hilbert space, inheriting inner product structure from $\ell^2(\N)$.

Mercer's theorem tells us that $H$ and $\Epsilon$ are isometrically isomorphic under the canonical linear map given by
$$
f = \sum_{n \in \N}\beta_n \phi_n \mapsto \left(\frac{\beta_n}{\sqrt{\mu_n}}\right)_{n \in \N}.
$$
Thus, studying functions in $H$ reduces to studying sequences whose components are given, loosely speaking, ``importance'' in proportion to $(\mu_n)_{n \in \N}$.

As a last point in this section, we discuss various rates of eigendecay for the sequences $(\mu_n)_{n\in\N}$ of eigenvalues associated with $k$, as this rate of decay effectively determines the ``size'' of $\Epsilon$. In particular, adopting terminology and definitions from \citet{vakili2021information}, we say the kernel $k$ experiences $(C, \beta)$-\textbf{polynomial eigendecay} for some $C> 0$ and $\beta> 1$ if the sequence of eigenvalues $(\mu_n)_{n \in \N}$ satisfies $\mu_n \leq C n^{-\beta}$ for all $n \in \N$. Correspondingly, we say $k$ experiences $(C_1, C_2, \beta)$-\textbf{exponential eigendecay} if the sequence of eigenvalues $(\mu_n)_{n \in \N}$ satisfies $\mu_n \leq C_1\exp\{-C_2 n^\beta\}$ for all $n \in \N$.

The eigendecay of the two early-mentioned families of translation-invariant kernels has been well-studied. In particular, it is known that, for any $\sigma > 0$, there exists constants $C_1, C_2 > 0$ independent of dimension $d$ such that eigenvalues $(\mu_n)_{n \in \N}$ of the squared-exponential kernel satisfy $(C_1, C_2, \frac{1}{d})$-exponential eigendecay, i.e. $\mu_n \leq C_1\exp\{-C_2 n^{1/d}\}$ \citep{belkin2018approximation, wainwright2019high, vakili2021information}. Likewise, for the Mat\'ern kernel, for any fixed smoothness $\nu > 1/2$ and bandwidth $\sigma > 0$, there is a constant $C > 0$ such that the corresponding eigenvalues $(\mu_n)_{n \in \N}$ satisfy $\left(C, \frac{2\nu + d}{d}\right)$-eigendecay, i.e. $\mu_n \leq Cn^{-\frac{2\nu + d}{d}}$~\citep{santin2016approximation, vakili2021information}. 


\subsection{Maximum Information Gain}

We now touch upon an important information-theoretic concept that, roughly, measures the complexity of a kernel function $k$. Let $f \sim \GP(0, k)$ be drawn from a Gaussian process on $\calX$ with mean function $m(x) = 0$ and covariance function given by the kernel $k$. For any finite set $A = \{x_1, \dots, x_n\} \subset \calX$, let $y_A$ be the length $n$ vector whose $i$th coordinate is given by $f(x_i) + \epsilon_i$, where $\epsilon_i \sim \calN(0, \rho)$ are independent and identically distributed. Likewise, let $f_A$ be the length $n$ vector whose $i$th coordinate is given by $f(x_i)$.

With these quantities, we can define the \textbf{information gain} associated with index set $A \subset \calX$ as the mutual information between $y_A$ and $f_A$, i.e. quantity
$$
I(y_A, f_A) = H(y_A) - H(y_A \mid f_A) = \frac{1}{2}\log\det(\id_H + \rho^{-1}M_A),
$$
where $id_H : H \rightarrow H$ is the identity operator on the RKHS $H$ associated with kernel $k$, and $A : H \rightarrow H$ is the finite-rank operator given by $M_A := \sum_{x \in A}k(\cdot, x)k(\cdot, x)^T = \sum_{x \in A}k(\cdot, x)(k(\cdot, x), \cdot)_H$. Since $M_A$ is of finite rank, $\det(\id_H + \rho^{-1}M_A)$ is well-defined in the sense of the Fredholm derminant --- that is as the product of the (finitely many) eigenvalues of the operator $\id_H + \rho^{-1}M_A$. Intuitively, the information gain measures how much about the noisy observations $y_A$ knowing the true function values $f_A$ reveals.

For those unfamiliar with the theory of Fredholm determinants, it can be readily checked that, letting $n := |A|$, we have
$$
\det(\id_H + \rho^{-1}M_A) = \det(I_n + \rho^{-1}K_A),
$$
where $I_n$ is the identity on $\R^n$ and $K_A$ is the Gram matrix given by $K = (k(x_i, x_j))_{i, j \in [n]}$. We prefer the use of the Fredholm determinant, however, as this quantity will allow us to more elegantly state our bounds in the sequel.

Given the above quantity of information, one could ask the question ``for any $T$, which $A \subset \calX$ of $|A| = T$ maximizes information gain?''. This motivates defining the \textbf{maximum information gain} of order $T$, which is the quantity defined as
$$
\gamma_T(\rho) := \max_{A \subset \calX : |A| = T}I(y_A, f_A) = \max_{A \subset \calX : |A| = T}\frac{1}{2}\log\det(\id_H + \rho^{-1}M_A)
$$
This naturally quantity turns out to not only be integral in characterizing upper bounds on regret in kernelized learning problems~\citep{chowdhury2017kernelized,janz2020bandit,vakili2021information,srinivas2009gaussian, valko2013finite}, but also in characterizing lower bounds on regret as well~\citep{janz2020bandit,scarlett2017lower}.

Before proceeding, we note a difference in our notation compared to existing works. In particular, we explicit note the dependence of tthe max information gain on the underlying noise or regularization parameter $\rho$. As we will shortly see, $\gamma_T(\rho)$ can readily be bounded both ass a function of the time-horizon $T$ and regularization parameter $\rho$. 

We characterize the rate of growth of $\gamma_T(\rho)$ for the two regimes of eigendecay outlined in the previous section: polynomial and exponential eigendecay. We additionally make the following assumption on the kernel $k$, which was introduced by \citet{vakili2021information}. 

\begin{ass}
\label{ass:kernel_struc}
We assume that the kernel function $k : \calX \times \calX \rightarrow \R$ satisfies (a) $|k(x, y)| \leq K$ for some $K > 0$ and all $x, y \in \calX$ and (b) $|\phi_m(x)| \leq \psi$ for some $\psi > 0$ and all $m \geq 1$, $x \in \calX$.

\end{ass}

In particular, we leverage the following result of \citet{vakili2021information}.

\begin{lemma}[Corollary 1 in \citet{vakili2021information}]
\label{lem:info_gain_bound}
Let $k : \calX \times \calX \rightarrow \R$ be a kernel function satisfying the assumptions of Theorem~\ref{thm:mercer}. Further assume that there exist $\psi, K > 0$ such that for all $x \in \calX$, $|k(x, x)| \leq K$ and for all $n \in \N$ and $x \in \calX$, $|\phi_n(x)| \leq \psi$. let $\gamma_T(\rho)$ be the max-information, as outlined above. The following hold.
\begin{enumerate}
\item If $k$ experiences $(C, \beta)$-polynomial eigendecay, then
$$
\gamma_T(\rho) \leq \left(\left(\frac{C\psi^2T}{\rho}\right)^{1/\beta}\log^{-1/\beta}\left(1 + \frac{KT}{\rho}\right) + 1 \right)\log\left(1 + \frac{KT}{\rho}\right).
$$
\item If $k$ experiences $(C_1, C_2, \beta)$-exponential eigendecay, then
$$
\gamma_T(\rho) \leq \left(\left(\frac{2}{C_2}\left(\log(T) + C_\beta\right)\right)^{1/\beta} + 1\right)\log\left(1 + \frac{KT}{\rho}\right)
$$
where $C_\beta = \log\left(\frac{C_1\psi^2}{C_2\rho}\right)$ if $\beta = 1$ and $C_\beta = \log\left(\frac{2C_1\psi^2}{\rho\beta C_2}\right) + \left(\frac{1}{\beta} - 1\right)\left(\log\left(\frac{2}{C_2}\left(\frac{1}{\beta} - 1\right)\right) - 1\right)$
\end{enumerate}

\end{lemma}

While the above bounds on maximum information gain are quite messy, they can be greatly simplified if we allow ourselves the use of bounding constants depending only on the kernel $k$ and not the time-horizon $T$ and the regularization parameter $\rho$. The following is also taken from \citet{vakili2021information}, but we have been careful to explicitly include the dependence on $\rho$ in the result.

\begin{corollary}
\label{cor:info_gain_bound}
Suppose $(k_d)_{d \geq 1}$ be a family of kernels (indexed by dimension $d$) such that, for each $d$, $k_d$ satisfies the assumptions of Lemma~\ref{lem:info_gain_bound} above with $\psi, K > 0$ also not depending on $d$. The following hold.
\begin{enumerate}
    \item If there is a constant $C > 0$ independent of $d$ such that $k_d$ experiences $(C, \beta_d)$-polynomial eigendecay, then
    $$
    \gamma_T(\rho) = O\left(\left(\frac{T}{\rho}\right)^{1/\beta_d}\log^{1 - \frac{1}{\beta_d}}\left(\frac{T}{\rho}\right)\right).
    $$
    \item If there are constants $C_1, C_2$ independent of $d$ such that $k_d$ experiences $(C_1, C_2, \beta_d)$-exponential eigendecay, then
    $$
    \gamma_T(\rho) = O\left(\log^{1 + \frac{1}{\beta}}\left(\frac{T}{\rho}\right)\right).
    $$.

    In particular, if $(k_d)_{d \geq 1}$ is the squared exponential family of kernels with bandwidth $\sigma > 0$, we have $\gamma_T(\rho) = O\left(\log^{d + 1}\left(\frac{T}{\rho}\right)\right)$. Note that this rate is independent of bandwidth $\sigma > 0$. Likewise, if $(k_d)_{d \geq 1}$ is a family of $(\nu, \sigma)$-Mat\'ern kernels, we have $\gamma_T(\rho) = O\left(\left(\frac{T}{\rho}\right)^{\frac{d}{2\nu + d}}\log^{\frac{2\nu}{2\nu + d}}\left(\frac{T}{\rho}\right)\right)$, where we note the asymptotics for $\gamma_T(\rho)$ in this case possess a dependence on $\nu$ but not on $\sigma$.
\end{enumerate}

\end{corollary}
  

==> old_tex/bandit_problem.tex <==
\section{Bandit Problem}

We now formally introduce the kernelized bandit problem. Fix some bounded $\calX \subset \R^d$, and let $k : \calX \times \calX \rightarrow \R$ be some kernel function. Let $(H, (\cdot, \cdot)_H)$ be the RKHS associated with $k$, and let $f^\ast \in H$ be some one unknown function satisfying $\|f^\ast\|_H \leq D$, where $D > 0$ is some known constant. Further, suppose that, for all $x \in \calX$, $\|k(\cdot, x)\|_H \leq B$, where $B > 0$ is some other known constant.

In the kernelized bandit problem, an agent sequentially interacts with an environment over $T > 0$ rounds in the following manner. At the start of each round $t \in [T]$, the agent selects a point $X_t \in \calX$ using the information acquired in previous rounds. The agent then observes a noisy response $Y_t := f^\ast(X_t) + \epsilon_t$, where $\epsilon_t$ is conditionally $\sigma$-subGaussian conditioned on previous observations, i.e. we have 
$$
\log\E\left(e^{\lambda \epsilon_t} \mid \calF_{t - 1}\right) \leq \frac{\lambda^2\sigma^2}{2} \quad \text{for all } \lambda \in \R,
$$
where $(\calF_t)_{t \geq 0}$ is the filtration given by $\calF_t := \sigma(Y_s : s \leq t)$. By convention, we assume $\sigma(\emptyset)$ is the trivial $\sigma$-algebra. Note that, under the aforementioned observation model, $(X_t)_{t \geq 0}$ can be viewed as an $(\calF_t)_{t \geq 0}$-predictable sequence of random elements of $\calX$. 

The goal of agent is to, with high probability, minimize the \textbf{regret at time $T$}, which is the random variable given by
\begin{align*}
R_T &:= \sum_{t = 1}^T\left\{f^\ast(x^\ast) - f^\ast(X_t)\right\}\\
&= \sum_{t = 1}^T\left\{ (f^\ast, k(\cdot, x^\ast))_H - (f^\ast, k(\cdot, X_t))_H\right\},
\end{align*}
where $x^\ast := \arg\min_{x \in \calX}f^\ast(x)$. In particular, the goal of the learner is to obtain \textbf{sublinear regret}, i.e. the agent desires $R_T = o(T)$ with high-probability.

In the case that the kernel experiences either polynomial or exponential eigendecay, as defined in the previous section, the following bounds are known on regret. In the case $k$ experiences $(C, \beta)$-polynomial eigendecay, it is known that there exists a policy for selecting $(X_t)_{t \geq 1}$ such that, with high-probability, $R_T = \widetilde{O}\left(T^{\frac{\beta + 1}{2\beta}}\right)$~\citep{valko2013finite, vakili2021information}. In the case of the $(\nu, \sigma)$-Mat\'ern kernel in dimension $d$, this reduces to a high-probability regret bound of $R_T = \widetilde{O}\left(T^{\frac{\nu + d}{2\nu + d}}\right)$, which is known to be tight~\citep{scarlett2017lower}. Likewise, in the case of $(C_1, C_2, \beta)$-exponential eigendecay, there are policies obtaining regret $R_T = \widetilde{O}\left(T^{1/2}\log^{\frac{1}{2\beta}}(T)\right)$~\citep{valko2013finite, vakili2021information}. For the $\sigma$-squared exponential kernel in dimension $d$, this gives a regret rate of $R_T = \widetilde{O}\left(T^{1/2}\log^{d/2}(T)\right)$, which is once again known to be tight~\citep{scarlett2017lower}.

Since the squared exponential and Mat\'ern kernels are amongst most commonly used, and since there are algorithms attaining the known lower bound on regret up to lower order terms, it may seem that the kernelized bandit problem is solved. However, the existing regret optimal algorithms are intricate and computationally expensive, relying on computing a careful, adaptive discretization of the input space $\calX$. The simplest algorithm, Gaussian Process Upper Confidence Bound, or GP-UCB, is computationally efficient and performs well in practice (see Algorithm~\ref{alg:UCB}). However, the best analysis of the performance of GP-UCB obtains regret $\widetilde{O}(\gamma_T\sqrt{T})$~\citep{chowdhury2017kernelized}, which, as noted by \citet{vakili2021information,vakili2021open}, can be super-linear when working with the Mat\'ern family of kernels. 

In this write up, we aim to show that the seemingly poor regret performance of GP-UCB is a product of existing analysis, and not a facet of the algorithm itself. In particular, in Section~\ref{} below, we offer an improved concentration bound for random elements in a reproducing kernel Hilbert space. Using these improved concentration bounds, we are able to significantly improve that regret bounds for GP-UCB, showing that the algorithm obtains almost optimal regret under polynomial and exponential eigendecay. 

\begin{algorithm}
\label{alg:UCB}
\caption{Gaussian Process Upper Confidence Bound}
\begin{algorithmic}
\Require $(U_t)_{t \geq 0}$ data-dependent confidence bounds, $\rho > 0$ regularization parameter, $T \in \N$ time horizon.
\Procedure{GP-UCB}{$(U_t)$, $\rho$, $T$}
\State $\Epsilon_1 \gets \left\{f \in H: \|f\|_H \leq D\right\}$
\State $V_0 := \rho\id_H$
\For{$t \in 1, \dots, T$}
    \State $X_t \gets \arg\max_{x \in \calX, f \in \Epsilon_t}f(x)$
    \State Agent plays $X_t$
    \State Agent observes reward $Y_t := f^\ast(X_t) + \epsilon_t$
    \State $V_t := V_{t - 1} + k(\cdot, X_t)k(\cdot, X_t)^T$
    \State $f_t := (V_t + \rho \id_H)^{-1}\Phi_t^T Y_{1:t}$
    \State $\Epsilon_{t + 1} \gets \left\{ f \in H : \|f\|_H \leq D, \left\|V_t^{1/2}(f - f_t)\right\|_H \leq U_t \right\}$

\EndFor
\Return


\EndProcedure
\end{algorithmic}
\end{algorithm}



==> old_tex/new_analysis.tex <==
\section{A New Analysis}
In this section, we provide a new analysis for the Gaussian process upper confidence bound (GP-UCB) algorithm. We take inspiration from the work of \citet{vakili2021information}, who use a truncation-based argument to bound the regret Let $n \geq 1$ be some arbitrary positive integer. The idea behind our analysis is to split the kernel $k$ into two kernels: one from projecting $k$ onto the $n$ most significant basis functions in the underlying RKHS, and another, orthogonal kernel from projecting $k$ onto the remaining basis functions. By studying the growth of regret $R_T$ with respect to the maximum information gain of the two component kernels and then optimizing over the truncation level $n$, we will show that GP-UCB actually obtains the lower bound on regret.

\begin{proof}


\begin{align*}
r_t &:= (f^\ast, k(\cdot, x^\ast))_H - (f^\ast, k(\cdot, X_t))_H \\
&\leq (\wt{f}_t, k(\cdot, X_t))_H - (f^\ast, k(\cdot, X_t))_H \\
&= (\wt{f}_t - f_t, k(\cdot, X_t))_H - (f_t - f^\ast, k(\cdot, X_t))_H\\
&= (\pi_n(\wt{f}_t - f_t), \pi_nk(\cdot, X_t))_H - (\pi_n(f_t - f^\ast), \pi_nk(\cdot, X_t))_H \\
&\qquad + (\pi_n^\perp(\wt{f}_t - f_t), \pi_n^\perp k(\cdot, X_t))_H - (\pi_n^\perp(f_t - f^\ast), \pi_n^\perp k(\cdot, X_t))_H \\
&= (\pi_n(\wt{f}_t - f_t), \pi_nk(\cdot, X_t))_{H_n} - (\pi_n(f_t - f^\ast), \pi_nk(\cdot, X_t))_{H_n} \\
&\qquad + (\pi_n^\perp(\wt{f}_t - f_t), \pi_n^\perp k(\cdot, X_t))_{H_n^\perp} - (\pi_n^\perp(f_t - f^\ast), \pi_n^\perp k(\cdot, X_t))_{H_n^\perp} \\
&= \left(V_{t, \parallel}^{1/2}\pi_n(\wt{f}_t - f_t), V_{t, \parallel}^{-1/2}\pi_nk(\cdot, X_t)\right)_{H_n} - \left(V_{t, \parallel}^{1/2}\pi_n(f_t - f^\ast), V_{t, \parallel}^{-1/2}\pi_nk(\cdot, X_t)\right)_{H_n} \\
&\qquad + \left(V_{t, \perp}^{1/2}\pi_n^\perp(\wt{f}_t - f_t), V_{t, \perp}^{-1/2}\pi_n^\perp k(\cdot, X_t)\right)_{H_n^\perp} - \left(V_{t, \perp}^{1/2}\pi_n^\perp(f_t - f^\ast), V_{t, \perp}^{-1/2}\pi_n^\perp k(\cdot, X_t)\right)_{H_n^\perp} \\
&\leq \left\|V_{t, \parallel}^{1/2}\pi_n(\wt{f}_t - f_t)\right\|_{H_n} \left\|V_{t, \parallel}^{-1/2}\pi_nk(\cdot, X_t)\right\|_{H_n} + \left\|V_{t, \parallel}^{1/2}\pi_n(f_t - f^\ast)\right\|_{H_n} \left\|V_{t, \parallel}^{-1/2}\pi_nk(\cdot, X_t)\right\|_{H_n} \\
&\qquad + \left\|V_{t, \perp}^{1/2}\pi_n^\perp(\wt{f}_t - f_t)\right\|_{H_n^\perp} \left\|V_{t, \perp}^{-1/2}\pi_n^\perp k(\cdot, X_t)\right\|_{H_n^\perp} + \left\|V_{t, \perp}^{1/2}\pi_n^\perp(f_t - f^\ast)\right\|_{H_n^\perp} \left\|V_{t, \perp}^{-1/2}\pi_n^\perp k(\cdot, X_t)\right\|_{H_n^\perp}.
\end{align*}
\end{proof}

\begin{algorithm}
\label{alg:UCB}
\caption{Split Upper Confidence Bound}
\begin{algorithmic}
\Require $\rho > 1$ regularization parameter, $T \in \N$ time horizon, $D$ bound on $\|f^\ast\|_H$, confidence parameter $\delta \in (0, 1)$, truncation level $n \geq 1$.
\Procedure{sUCB}{$\rho$, $T$, $D$, $\delta$, $n$}
\State $\Epsilon_0^\parallel := \left\{f \in H_n: \|f\|_{H_n} \leq D\right\}$, $\Epsilon_0^\perp := \left\{f \in H_n^\perp : \|f\|_{H_n^\perp} \leq D\right\}$
\State $V_{0, \parallel} := \rho \id_{H_n}$, $V_{0, \perp} := \rho \id_{H_n^\perp}$
\For{$t \in 1, \dots, T$}
    \State Agent plays $X_t := \arg\max_{x \in \calX} \max_{f^\parallel \in \Epsilon_{t - 1}^\parallel, f^\perp \in \Epsilon_{t - 1}^\perp}(f^\parallel + f^\perp)(x)$
    \State Agent observes reward $Y_t := f^\ast(X_t) + \epsilon_t$
    \State $V_{t, \parallel} := V_{t - 1, \parallel} + (\pi_nk(\cdot, X_t))(\pi_nk(\cdot, X_t))^T$
    \State $V_{t, \perp} := V_{t - 1, \perp} + (\pi_n^\perp k(\cdot, X_t))(\pi_n^\perp k(\cdot, X_t))^T$
    \State $f_t^\parallel := V_{t, \parallel}^{-1}\Phi_{t, \parallel}^T Y_{1:t}$
    \State $f_t^\perp := V_{t, \perp}^{-1}\Phi_{t, \perp}^T Y_{1:t}$
    \State $\Epsilon_t^{\parallel} := \left\{f \in H : \left\|V_{t, \parallel}^{1/2}\pi_n(f - f_t)\right\|_{H_n} \leq \sqrt{2\log\left(\frac{2}{\delta}\sqrt{\det(\rho^{-1}V_{t, \parallel})} \right)} + \rho^{1/2}D\right\}.$
    \State $\Epsilon_t^{\perp} := \left\{f \in H : \left\|V_{t, \perp}^{1/2}\pi_n^\perp(f - f_t)\right\|_{H_n^\perp} \leq \sqrt{2\log\left(\frac{2}{\delta}\sqrt{\det(\rho^{-1}V_{t, \perp})}\right)} + \rho^{1/2}D \right\}.$

\EndFor
\Return


\EndProcedure
\end{algorithmic}
\end{algorithm}

For fixed $n \geq 1,$ $t \in [T]$, and $(\calF_t)_{t \geq 0}$-predictable bounds 



\begin{lemma}
For a fixed truncation level $n \geq 1$, time horizon $T \geq 1$, and confidence level $\delta \in (0, 1)$, define the confidence ellipsoids $\Epsilon_t^{\parallel}, \Epsilon_t^{\perp} \subset H$ by
$$
\Epsilon_t^{\parallel} := \left\{f \in H : \left\|V_{t, \parallel}^{1/2}\pi_n(f - f_t)\right\|_{H} \leq \sqrt{2\log\left(\frac{2}{\delta}\sqrt{\det(\rho^{-1}V_{t, \parallel})} + \rho^{1/2}D\right)}\right\}
$$
and
$$
\Epsilon_t^{\perp} := \left\{f \in H : \left\|V_{t, \perp}^{1/2}\pi_n^\perp(f - f_t)\right\|_{H} \leq \sqrt{2\log\left(\frac{2}{\delta}\sqrt{\det(\rho^{-1}V_{t, \perp})}\right)} + \rho^{1/2}D \right\}. 
$$
Further define the confidence sets $(\Epsilon_t)_{t \geq 0}$ by $\Epsilon_t:= \Epsilon_{t}^{\parallel} \cap \Epsilon_t^{\perp}$. Then, we have 
$$
\P\left(\exists t \geq 1 : f^\ast \notin \Epsilon_t\right) \leq \delta.
$$
\end{lemma}

\begin{proof}
    Let $\square \in \{\parallel, \perp\}$, and let $\pi^{\parallel}_n := \pi_n$. First, observe that, using a standard argument, we have the decomposition
    \begin{align*}
    f_t - f^\ast &= (\Phi_t^T\Phi_t + \rho\id_H)^{-1}\Phi_t^TY_{1:t} - f^\ast \\
    &= (\Phi_t^T\Phi_t + \rho\id_H)^{-1}\Phi_t^T(\Phi_t f^\ast + \epsilon_{1:t}) - f^\ast \\
    &= (\Phi_t^T\Phi_t + \rho \id_H)^{-1}\Phi_t^T\epsilon_{1:t} - \rho(\Phi_t^T\Phi_t + \rho\id_H)^{-1}f^\ast \\
    &= V_t^{-1}\Phi_t^T\epsilon_{1:t} - \rho V_t^{-1}f^\ast.
    \end{align*}
\end{proof}

{\color{red} $\square$ only defined within proof. define below.}

For a linear operator $A : H \rightarrow H$, let $A^+$ denote the Moore-Penrose pseudo-inverse. When $A$ is a projection operator, we know that $A^+ = A$. We have the identity $\pi_n^\square V_t^{-1} = \left(\pi_n^\square\right)^+V_t^{-1} = \left[V_t \pi_n^\square\right]^+ = V_{t, \square}^+$. Thus, we can write
$$
\pi_n(f_t - f^\ast) = \pi_nV_t^{-1}\Phi_t^T\epsilon_{1:t} - \rho V_t^{-1}f^\ast = V_{t, \square}^{+}\Phi_t^T\epsilon_{1:t} - \rho V_{t, \square}^{+}f^\ast.
$$

Now, let $g \in H_n^{\square} \subset H$ be arbitrary. We have 
\begin{align*}
\left(g, \pi_n^\square(f_t - f^\ast)\right)_{H} &= \left(\pi_n^\square g, \pi_n^\square(f_t - f^\ast)\right)_H \\
&= \left(\pi_n^\square g, V_{t, \square}^{+}\Phi_t^T\epsilon_{1:t}\right)_H - \rho\left(\pi_n^{\square} g , V_{t, \square}^+ f^\ast\right)_H
\end{align*}


\begin{theorem}
Let $T > 0$ be a fixed time horizon and $\rho > 1$ an arbitrary truncation level. Then, Algorithm~\ref{alg:UCB} run with inputs $T, \rho,$ and confidence bounds $(U_t)_{t = 1}^T, T,$

\end{theorem}

\begin{proof}
For $t \in [T]$, define the linear operators $V_{t, \parallel} : H_n \rightarrow H_n$ and $V_{t, \perp} : H_n^\perp \rightarrow H_n^\perp$ (which implicitly depend on truncation level $n$) by
$$
V_{t, \parallel} := \sum_{s = 1}^t(\pi_n k(\cdot, X_s))(\pi_n k(\cdot, X_s))^T + \rho I_n \quad V_{t, \perp} := \sum_{s = 1}^t(\pi_n^\perp k(\cdot, X_s))(\pi_n^\perp k(\cdot, X_s))^T + \rho \id_{H_n^\perp}.
$$


Observe that we can write the instantaneous regret as
\begin{align*}
r_t &:= (f^\ast, k(\cdot, x^\ast))_H - (f^\ast, k(\cdot, X_t))_H \\
&\leq (\wt{f}_t, k(\cdot, X_t))_H - (f^\ast, k(\cdot, X_t))_H \\
&= (\wt{f}_t - f_t, k(\cdot, X_t))_H - (f_t - f^\ast, k(\cdot, X_t))_H\\
&= (\pi_n(\wt{f}_t - f_t), \pi_nk(\cdot, X_t))_H - (\pi_n(f_t - f^\ast), \pi_nk(\cdot, X_t))_H \\
&\qquad + (\pi_n^\perp(\wt{f}_t - f_t), \pi_n^\perp k(\cdot, X_t))_H - (\pi_n^\perp(f_t - f^\ast), \pi_n^\perp k(\cdot, X_t))_H \\
&= (\pi_n(\wt{f}_t - f_t), \pi_nk(\cdot, X_t))_{H_n} - (\pi_n(f_t - f^\ast), \pi_nk(\cdot, X_t))_{H_n} \\
&\qquad + (\pi_n^\perp(\wt{f}_t - f_t), \pi_n^\perp k(\cdot, X_t))_{H_n^\perp} - (\pi_n^\perp(f_t - f^\ast), \pi_n^\perp k(\cdot, X_t))_{H_n^\perp} \\
&= \left(V_{t, \parallel}^{1/2}\pi_n(\wt{f}_t - f_t), V_{t, \parallel}^{-1/2}\pi_nk(\cdot, X_t)\right)_{H_n} - \left(V_{t, \parallel}^{1/2}\pi_n(f_t - f^\ast), V_{t, \parallel}^{-1/2}\pi_nk(\cdot, X_t)\right)_{H_n} \\
&\qquad + \left(V_{t, \perp}^{1/2}\pi_n^\perp(\wt{f}_t - f_t), V_{t, \perp}^{-1/2}\pi_n^\perp k(\cdot, X_t)\right)_{H_n^\perp} - \left(V_{t, \perp}^{1/2}\pi_n^\perp(f_t - f^\ast), V_{t, \perp}^{-1/2}\pi_n^\perp k(\cdot, X_t)\right)_{H_n^\perp} \\
&\leq \left\|V_{t, \parallel}^{1/2}\pi_n(\wt{f}_t - f_t)\right\|_{H_n} \left\|V_{t, \parallel}^{-1/2}\pi_nk(\cdot, X_t)\right\|_{H_n} + \left\|V_{t, \parallel}^{1/2}\pi_n(f_t - f^\ast)\right\|_{H_n} \left\|V_{t, \parallel}^{-1/2}\pi_nk(\cdot, X_t)\right\|_{H_n} \\
&\qquad + \left\|V_{t, \perp}^{1/2}\pi_n^\perp(\wt{f}_t - f_t)\right\|_{H_n^\perp} \left\|V_{t, \perp}^{-1/2}\pi_n^\perp k(\cdot, X_t)\right\|_{H_n^\perp} + \left\|V_{t, \perp}^{1/2}\pi_n^\perp(f_t - f^\ast)\right\|_{H_n^\perp} \left\|V_{t, \perp}^{-1/2}\pi_n^\perp k(\cdot, X_t)\right\|_{H_n^\perp}.
\end{align*}

For any operator $A : H \rightarrow H$ and a subspace $H' \subset H$, we let $A|_{H'} : H' \rightarrow H$ denote the restriction of $A$ to subspace $H'$. Recall that we have defined $H_n := \spn\left(\left\{\varphi_1, \dots, \varphi_n\right\}\right)$ to be the span of the first $n$ renormalized basis functions associated with kernel $k$, and $H_n^{\perp}$ to be the orthogonal complement of $H_n$ in $H$ with respect to the inner product $(\cdot, \cdot)_H$. 

Observe that, by construction, $V_{t, \parallel}$ sends elements of $H_n$

Applying 

\end{proof}



Observe that we have, with probability at least $1 - \delta$
\begin{align*}
r_t &= (f^\ast, k(\cdot, x^\ast))_H - (f^\ast, k(\cdot, X_t))_H \\
&\leq (\wt{f}_t, k(\cdot, X_t))_H - (f^\ast, k(\cdot, X_t))_H \\
&= (\wt{f}_t - f_t, k(\cdot, X_t))_H - (f_t - f^\ast, k(\cdot, X_t))_H\\
&= (\pi_n(\wt{f}_t - f_t), \pi_n

\end{align*}




==> old_tex/truncated_kernel.tex <==
\section{Improved Regret by Kernel Truncation}

In this section, we introduce a new variation on the classic GP-UCB algorithm that obtains improved regret over the original version. At a high level, this variant of the UCB algorithm works by truncating the underlying kernel $k$ onto its $n$ most significant components, where $n$ is determined based on (a) the time horizon $T$ and (b) the underlying smoothness of the kernel $k$, which is linked to its rate of eigendecay.

Recall that $(\varphi_m)_{m \geq 1} := (\sqrt{\mu_m}\phi_m)_{m \geq 1}$ forms an orthonormal basis for the space $(H, (\cdot, \cdot)_H)$, and that $H$ can be represented as
$$
H := \left\{f = \sum_{m = 1}^\infty\theta_m\varphi_m : \sum_{m = 1}^\infty \theta_m^2 < \infty\right\}.
$$
Let $(H_n, (\cdot, \cdot)_n)$ be the truncated Hilbert space given by
$$
H_n := \left\{f = \sum_{m = 1}^n\theta_m\varphi_m\right\} \qquad (f, g)_n = (f, g)_H, \text{ for } f, g\in H_n.
$$
It can be checked that $(H_n, (\cdot, \cdot)_n)$ is also a RKHS, with associated kernel $k_n(x, y) := (\pi_n k(\cdot, x), \pi_n k(\cdot, y))_n = (\pi_n k(\cdot, x), \pi_n k(\cdot, y))_H$, where $\pi_n : H \rightarrow H_n$ is the natural projection given by
$\pi_nf = \sum_{m = 1}^n(f, \varphi_m)_H\varphi_m$.


Observe that, for any $n \geq 1$, we can decompose the regret up to time $T > 0$ as
\begin{align*}
R_T &= \sum_{t = 1}^T\left\{(f^\ast, k(\cdot, x^\ast))_H - (f^\ast, k(\cdot, k(\cdot, X_t))_H\right\} \\
&= \sum_{t = 1}^T\left\{(\pi_n f^\ast, \pi_nk(\cdot, x^\ast))_H - (\pi_n f^\ast, \pi_nk(\cdot, X_t))_H\right\} + \sum_{t = 1}^T\left\{(\pi_n^\perp f^\ast, \pi_n^\perp k(\cdot, x^\ast))_H - (\pi_n^\perp f^\ast, \pi_n^\perp k(\cdot, X_t))\right\} \\
&=\sum_{t = 1}^T\left\{(\pi_n f^\ast, k_n(\cdot, x^\ast))_n - (\pi_n f^\ast, k_n(\cdot, X_t))_n\right\} + \sum_{t = 1}^T\left\{(\pi_n^\perp f^\ast, \pi_n^\perp k(\cdot, x^\ast))_H - (\pi_n^\perp f^\ast, \pi_n^\perp k(\cdot, X_t))\right\} \\
&=: R_T^{\parallel}(n) + R_T^{\perp}(n).
\end{align*}

We focus on bounding these terms separately for an arbitrary level of truncation $n \geq 1$. After doing this analysis, we will then be able to optimize over choice of $n$ to obtain our desired regret bounds.

\begin{lemma}
\label{lem:perp_reg_bound}
Let $n \geq 1$ be an arbitrary truncation level, and $T > 1$ an arbitrary time horizon. Further, let $R_T^\perp(n)$ be the perpendicular regret, as defined above. Then, we have the bound
\begin{equation}
    \label{bd:gen_perp_bd}
    R_T^\perp(n) \leq 2T\psi\|f^\ast\|_H\sqrt{\sum_{m = n + 1}^\infty \mu_m}.
\end{equation}
In particular, if the kernel $k$ experiences $(C, \beta)$-polynomial eigendecay, we have 
\begin{equation}
\label{bd:poly_perp_bd}
R_T^\perp(n) \leq 2T\psi\sqrt{C}\sqrt{n^{1 - \beta}}.
\end{equation}


\end{lemma}

\begin{proof}
Observe that we have the bound
\begin{align*}
R_T^{\perp}(n) &= \sum_{t = 1}^T\left\{(\pi_n^\perp f^\ast, \pi_n^\perp k(\cdot, x^\ast))_H - (\pi_n^\perp f^\ast, \pi_n^\perp k(\cdot, X_t))_H\right\} \\
&\leq \|\pi_n^\perp f^\ast\|_H\sum_{t = 1}^T\|\pi_n^\perp(k(\cdot, x^\ast) - k(\cdot, X_t))\|_H \\
&\leq 2T\|f^\ast\|_H\sup_{x \in \calX}\|\pi_n^\perp k(\cdot, x)\|_H
\end{align*}

Next, observe that, for any fixed $x \in \calX$, we have
$$
\pi_n^\perp k(\cdot, x) = \sum_{m = n + 1}^\infty \mu_m \phi_m(x) \phi_m.
$$
Thus, evaluating the lefthand side under the squared RKHS norm gives
$$
\|\pi_n^\perp k(\cdot, x)\|^2_H = \sum_{m = n + 1}^\infty \mu_m|\phi_m(x)|^2 \leq \sum_{m = n + 1}^\infty \mu_m \psi^2,
$$
where the first inequality follows from condition (b) of Assumption~\ref{ass:kernel_struc}. Consequently, since this final righthand side bound is independent of the choice of $x \in \calX$, we have
$$
R_T^\perp(n) \leq 2T\psi\|f^\ast\|_H  \sqrt{\sum_{m = n + 1}^\infty \mu_m},
$$
which proves the perpendicular regret bound in Bound~\ref{bd:gen_perp_bd}. Now, observe that under the assumption of $(C, \beta)$-polynomial eigendecay, we have
\begin{align*}
\sum_{m = n + 1}^\infty \mu_m &\leq \sum_{m = n + 1}^\infty Cm^{-\beta} \\
&\leq C\int_{n}^\infty z^{-\beta}dz\\
&\leq Cn^{1 - \beta}.
\end{align*}
Thus, plugging this into the generic perpendicular regret bound, we have
$$
R_T^{\perp}(n) \leq 2C^{1/2}T\psi\|f^\ast\|_H\sqrt{n^{1 - \beta}},
$$
proving the bound in Inequality~\ref{bd:poly_perp_bd}.


\end{proof}

We now turn towards bounding the parallel regret $R_T^{\parallel}(n)$. We first start by constructing a truncated version of our confidence ellipsoids

\begin{lemma}[Truncated Max-Information Gain]
Let $k : \calX \times \calX \rightarrow \R$ be a kernel satisfying Assumption~\ref{ass:kernel_struc} and let $n \geq 1$ be an arbitrary truncation level. Let $k_n := \pi_n k$ be the truncated kernel onto the first $n$ orthonormal basis elements. For $\rho, T > 1$, let $\gamma_T^{(n)}(\rho)$ be the maximum-information gain associated with $k_n$, i.e.
\begin{align*}
\gamma_T^{(n)}(\rho) &= \frac{1}{2}\max_{x_1, \dots, x_T \in \calX}\log\det\left(I_n + \rho^{-1}\sum_{t = 1}^Tk_n(\cdot, x_t)k_n(\cdot, x_t)^T\right) \\
&= \frac{1}{2}\max_{x_1, \dots, x_T \in \calX}\log\det\left(\id_H + \rho^{-1}\sum_{t = 1}^T\pi_nk(\cdot, x_t)(\pi_n k(\cdot, x_t))^T\right).
\end{align*}
We have the bound
$$
\gamma_T^{(n)}(\rho) \leq \frac{1}{2}n\log\left(1 + \frac{TK}{\rho n}\right).
$$

\end{lemma}

\begin{proof}
Fix $x_1, \dots, x_T \in \calX$. Recall that, for any positive-definite matrix $A$, we have the bound
$$
\log\det A \leq n\log\left(\frac{\Tr A}{n}\right).
$$
Thus, we have 
\begin{align*}
&\log\det\left(I_n + \rho^{-1}\sum_{t = 1}^Tk_n(\cdot, x_t)k(\cdot, x_t)^T\right) \\
&\leq n\log\left(\frac{1}{n}\Tr \left( I_n + \rho^{-1}\sum_{t = 1}^Tk_n(\cdot, x_t)k(\cdot, x_t)^T\right)\right)\\
&= n\log\left(1 + \frac{1}{\rho}\sum_{t = 1}^T\Tr\left[k_n(\cdot, x_t)k(\cdot, x_t)^T\right]\right) \\
&= n\log\left(1 + \frac{1}{\rho n}\sum_{t  = 1}^T\|k_n(\cdot, x_t)\|_H^2\right) \\ 
&\leq n\log\left(1 + \frac{TK}{\rho n}\right).
\end{align*}
Notice that the final bound is independent of the sequence of chosen points $x_1, \dots, x_T \in \calX$. Thus, taking the supremum over all such sequences and dividing by two yields
$$
\gamma_T^{(n)}(\rho) \leq \frac{n}{2}\log\left(1 + \frac{TK}{\rho n}\right),
$$
which proves the desired result.
\end{proof}

\begin{lemma}[Truncated Confidence Ellipsoids]
Let $(X_t)_{t \geq 1}$ be an $(\calF_t)_{t \geq 0}$-predictable sequence of $\calX$-valued random variables, where we recall $\calF_t := \sigma(\epsilon_s : s \leq t)$. Let $f^\ast \in H$ satisfy $\|f^\ast\|_H \leq D$. Let $(Y_t)_{t \geq 0}$ be the $(\calF_t)_{t \geq 0}$-adapted sequence of response variables given by
$$
Y_t := f^\ast(X_t) + \epsilon_t = (f^\ast, k(\cdot, X_t))_H + \epsilon_t.
$$
Define the sequence of truncated ridge estimators $(f^{(n)}_t)_{t \geq 1}$ by

\begin{align*} 
f^{(n)}_t &:= \left(\sum_{s \leq t}k_n(\cdot, X_s)k_n(\cdot, X_s)^T + \rho\id_H\right)^{-1}\Phi_t(n)^TY_{1:t}
\end{align*}
where $\Phi_t(n) := (k_n(\cdot, X_1), \dots, k_n(\cdot, X_t))^T$ and $Y_{1:t} := (Y_1, \dots, Y_t)^T$.

Then, with probability at least $1 - \delta$, simultaneously for all $t \geq 1$ we have
\begin{align*}
\left\|V_t(n)^{-1/2}\left(f^{(n)}_t - \pi_n f^\ast\right)\right\| &\leq \sqrt{2\log\left(\frac{1}{\delta}\sqrt{\det(\id_H + \rho^{-1}V_t(n)}\right)} + \rho^{1/2}D\\
&\leq \sqrt{2(\gamma_T^{(n)}(\rho) + \log(1/\delta))} + \rho^{1/2}D.
\end{align*}

\end{lemma}

\begin{proof}
    
\end{proof}

\begin{lemma}
\label{lem:par_reg_bd}

\end{lemma}

\begin{proof}
    For $t \in [T]$, define the instantaneous parallel regret $r_t^{\parallel}(n)$ by
    \begin{align*}
    r_t^{\parallel}(n) &:= (\pi_n f^\ast, \pi_n k(\cdot, x^\ast))_H - (\pi_n f^\ast, \pi_n k(\cdot, X_t))_H \\ 
    &\leq (\pi_n \widetilde{f}_t, k(\cdot, X_t))_H + 

    \end{align*}
\end{proof}

